Multiobjective Preexpectation Reasoning for Probabilistic Programs

Probabilistic programs with nondeterminism model planning problems in which a strategy typically resolves the nondeterminism to meet a specification. We study the multiobjective setting, meeting several specifications at once along a Pareto front, and provide a deductive, program-level account of strategy synthesis. Its core is a multiobjective preexpectation transformer mapping a tuple of postexpectations to the set of simultaneously achievable values, an element of the convex Hoare powerdomain. It conservatively extends weakest preexpectations and lifts standard loop rules. We develop rules to synthesize witnessing strategies as mixed determinizations that solve nondeterminism probabilistically. We prove the transformer and synthesis rules sound against an operational Markov decision process (MDP) semantics, without requiring a finite state space: our approach can be seen as a symbolic approach - at program level - for multiobjective optimization over infinite MDPs. We demonstrate our machinery using two case studies.

==> macros.tex <==
\makeatletter
\DeclareFontFamily{U}{MnSymbolA}{}

\DeclareFontShape{U}{MnSymbolA}{m}{n}{
    <-6>  MnSymbolA5
   <6-7>  MnSymbolA6
   <7-8>  MnSymbolA7
   <8-9>  MnSymbolA8
   <9-10> MnSymbolA9
  <10-12> MnSymbolA10
  <12->   MnSymbolA12}{}

\DeclareFontShape{U}{MnSymbolA}{b}{n}{
    <-6>  MnSymbolA-Bold5
   <6-7>  MnSymbolA-Bold6
   <7-8>  MnSymbolA-Bold7
   <8-9>  MnSymbolA-Bold8
   <9-10> MnSymbolA-Bold9
  <10-12> MnSymbolA-Bold10
  <12->   MnSymbolA-Bold12}{}

\DeclareSymbolFont{MnSymbolAonly}{U}{MnSymbolA}{m}{n}
\SetSymbolFont{MnSymbolAonly}{bold}{U}{MnSymbolA}{b}{n}

\DeclareMathSymbol{\uprsquigarrow}{\mathrel}{MnSymbolAonly}{"A9}
\newcommand{\uprsquigarrowbar}{\overline{\raisebox{2pt}{$\uprsquigarrow$}}}

\newcommand{\overuprsquigarrow}{%
  \mathrel{\raisebox{-.32ex}{$\overline{\smash{\raisebox{.32ex}{$\uprsquigarrow$}}\vphantom{\uprsquigarrow}}$}}%
}
\makeatother


\DeclarePairedDelimiter{\setBrace}{\{}{\}}
\DeclarePairedDelimiter{\paren}{(}{)}
\newcommand{\set}[1]{\ensuremath{\setBrace*{#1}}}


\newcommand{\dwcset}[1]{\ensuremath{\dwcNo\set{#1}}}
\newcommand{\dwcsetcomp}[2]{\ensuremath{\dwcNo\setcomp{#1}{#2}}}
\newcommand{\dwc}[1]{\ensuremath{\mathsf{dwc}\paren*{#1}}} %
\newcommand{\dwcNo}{\ensuremath{\mathsf{dwc}}}
\newcommand{\conv}[1]{\ensuremath{\mathsf{conv}\paren*{#1}}}
\newcommand{\convNo}{\ensuremath{\mathsf{conv}}}
\newcommand{\convset}[1]{\ensuremath{\convNo\set{#1}}}
\newcommand{\convsetcomp}[2]{\ensuremath{\convNo\setcomp{#1}{#2}}}
\newcommand{\cl}[1]{\ensuremath{\mathsf{cl}\paren*{#1}}}%

\newcommand{\clopen}[1]{\ensuremath{\mathsf{cl}({#1}}} %
\newcommand{\convopen}[1]{\ensuremath{\mathsf{conv}({#1}}} %


\newcommand{\todoin}[1]{\todo[inline]{#1}}
\newcommand{\sectiongoal}[1]{\todo[inline,color=black!10,author=Point of this section]{#1}\xspace}


\definecolor{hmcolor}{rgb}{0.42, 0.82, 0.91}
\newcommand{\hmcomment}[1]{\todo[color=hmcolor!70,size=\scriptsize,fancyline]{\textbf{HM}: #1}\xspace}
\newcommand{\hmcommentinline}[1]{\todo[inline,color=hmcolor!70,size=\small]{\textbf{HM}: #1}\xspace}
\newcommand{\hm}[1]{\hmcomment{#1}}
\newcommand{\hmin}[1]{\hmcommentinline{#1}}
\newcommand{\athm}{\colorbox{hmcolor!70}{\textbf{@Hannah}}}
\definecolor{lvcolor}{rgb}{0.82, 0.62, 0.91}
\newcommand{\lvcomment}[1]{\todo[color=lvcolor!70,size=\scriptsize,fancyline]{\textbf{LV}: #1}\xspace}
\newcommand{\lvcommentinline}[1]{\todo[inline,color=lvcolor!70,size=\small]{\textbf{LV}: #1}\xspace}
\newcommand{\lv}[1]{\lvcomment{#1}}
\newcommand{\lvin}[1]{\lvcommentinline{#1}}
\newcommand{\atlv}{\colorbox{lvcolor!70}{\textbf{@Lena}}}
\definecolor{kbcolor}{rgb}{0.5, 0.8, 1}
\newcommand{\kbcomment}[1]{\todo[color=kbcolor!70,size=\scriptsize,fancyline]{\textbf{KB}: #1}\xspace}
\newcommand{\kbcommentinline}[1]{\todo[inline,color=kbcolor!70,size=\small]{\textbf{KB}: #1}\xspace}
\newcommand{\kb}[1]{\kbcomment{#1}}
\newcommand{\kbin}[1]{\kbcommentinline{#1}}
\newcommand{\atkb}{\colorbox{kbcolor!70}{\textbf{@Kevin}}}
\definecolor{sjcolor}{rgb}{0.8, 1, 0.5}
\newcommand{\sjcomment}[1]{\todo[color=sjcolor!70,size=\scriptsize,fancyline]{\textbf{SJ}: #1}\xspace}
\newcommand{\sjcommentinline}[1]{\todo[inline,color=sjcolor!70,size=\small]{\textbf{SJ}: #1}\xspace}
\newcommand{\sj}[1]{\sjcomment{#1}}
\newcommand{\sjin}[1]{\sjcommentinline{#1}}
\newcommand{\atsj}{\colorbox{sjcolor!70}{\textbf{@Sebastian}}}
\colorlet{blkcolor}{orange}
\newcommand{\blkcomment}[1]{\todo[color=blkcolor!70,size=\scriptsize,fancyline]{\textbf{BLK}: #1}\xspace}
\newcommand{\blkcommentinline}[1]{\todo[inline,color=blkcolor!70,size=\small]{\textbf{BLK}: #1}\xspace}
\newcommand{\blk}[1]{\blkcomment{#1}}
\newcommand{\blkin}[1]{\blkcommentinline{#1}}
\newcommand{\atblk}{\colorbox{blkcolor!70}{\textbf{@Benjamin}}}
\colorlet{jpkcolor}{orange}
\newcommand{\jpkcomment}[1]{\todo[color=jpkcolor!70,size=\scriptsize,fancyline]{\textbf{JPK}: #1}\xspace}
\newcommand{\jpkcommentinline}[1]{\todo[inline,color=jpkcolor!70,size=\small]{\textbf{JPK}: #1}\xspace}
\newcommand{\jpk}[1]{\jpkcomment{#1}}
\newcommand{\jpkin}[1]{\jpkcommentinline{#1}}
\newcommand{\atjpk}{\colorbox{jpkcolor!70}{\textbf{@JPK}}}

\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\Q}{\ensuremath{\mathbb{Q}}}
\newcommand{\Nats}{\ensuremath{\mathbb{N}}\xspace}
\newcommand{\PosNats}{\ensuremath{\mathbb{N}_{>0}}\xspace}
\newcommand{\Ints}{\ensuremath{\mathbb{Z}}\xspace}
\newcommand{\Rats}{\ensuremath{\mathbb{Q}}\xspace}
\newcommand{\Reals}{\mathbb{R}}
\newcommand{\PosReals}{\mathbb{R}_{\geq 0}}
\newcommand{\PosRats}{\mathbb{Q}_{\geq 0}}
\newcommand{\PosRealsInf}{\overline{\mathbb{R}}_{\geq 0}}
\newcommand{\PosRealsInfVect}{\PosRealsInf^{\,n}}
\newcommand{\PosRealsVect}{\PosReals^n}
\newcommand{\minfty}{{-}\infty}
\newcommand{\pinfty}{{+}\infty}
\newcommand{\Rinf}{\ensuremath{\R^{{\pm}\infty}}}
\newcommand{\Powerset}[1]{\ensuremath{\mathcal{P}\paren*{#1}}}
\newcommand{\PowerDown}[1]{\ensuremath{\mathcal{P}_\downarrow\paren*{#1}}}
\newcommand{\DownSet}[1]{\ensuremath{\dwc{#1}}}
\newcommand{\HoarePower}[1]{\ensuremath{\PowerDown{#1}}}
\newcommand{\HoarePowerDom}{\ensuremath{\mathcal{H}}}
\newcommand{\MVdom}{\ensuremath{\HoarePowerDom}}
\newcommand{\MVset}{\ensuremath{\mathcal{V}}}
 
\newcommand{\A}{\mathbb{A}}
\newcommand{\B}{\mathbb{B}}

\newcommand{\labtau}{\tau}
\newcommand{\labalpha}{\alpha}
\newcommand{\labbeta}{\beta}
\newcommand{\Term}{\ensuremath{\Downarrow}}
\newcommand{\aexpr}{\ee}
\newcommand{\pexpr}{\ps}
\newcommand{\expsubs}[3]{{#1}[{#2} {{}\mapsto{}} {#3}]} %
\newcommand{\statesubst}[2]{[ #1 \mapsto #2 ]}
\newcommand{\ExecAbbr}[4]{\ensuremath{#1 \,\xrightarrow{{#2, #3}}\, #4 }}
\newcommand{\ExecAbbrSmash}[4]{\ensuremath{#1 \,\xrightarrow{\smash{#2, #3}}\, #4 }}
\newcommand{\actlab}{\ell}
\newcommand{\pnum}{q}
\newcommand{\TRUE}{\ttsymbol{{true}}}
\newcommand{\FALSE}{\ttsymbol{false}}
\newcommand{\true}{\TRUE}
\newcommand{\false}{\FALSE}
\newcommand{\trueBold}{\ttsymbol{\textbf{true}}}
\newcommand{\falseBold}{\ttsymbol{\textbf{false}}}

\newcommand{\pGCL}{\textnormal{\textsf{pGCL}}\xspace}   %
\newcommand{\Vars}{\ensuremath{\mathsf{Vars}}\xspace}   %
\newcommand{\VarsDom}{\ensuremath{\PosRats}}   %
\newcommand{\States}{\ensuremath{\Sigma}}
\newcommand{\iverson}[1]{\ensuremath{[#1]}}
\newcommand{\pstate}{\ensuremath{\sigma}}

\newcommand{\program}{\ensuremath{C}}
\newcommand{\guard}{\ensuremath{\varphi}} %
\newcommand{\ee}{\ensuremath{e}} %
\newcommand{\een}{\ensuremath{\boldsymbol{e}}} %

\newcommand{\SKIP}{\ttsymbol{skip}}
\newcommand{\REWARD}[1]{\ttsymbol{reward}\paren*{#1}}
\newcommand{\DIVERGE}{\ensuremath{\textnormal{\texttt{diverge}}}}

\newcommand{\AssignSymbol}{\coloneqq}
\newcommand{\ASSIGN}[2]{\ensuremath{#1 \AssignSymbol #2}}

\newcommand{\SEMI}{\ensuremath{\,;\,}}
\newcommand{\COMPOSE}[2]{\ensuremath{{#1}{\,\fatsemi}~ {#2}}}
\newcommand{\PCHOICE}[3]{\ensuremath{\left\{\, {#1} \,\right\}\mathrel{\left[\,#2\,\right]}\left\{\, {#3} \,\right\}}}
\newcommand{\NDCHOICE}[2]{\ensuremath{\left\{\, {#1} \,\right\}\mathrel{\Box}\left\{\, {#2} \,\right\}}}
\newcommand{\NDBRACK}{\ensuremath{\left.\right\}\mathrel{\Box}\left\{\right.}}
\newcommand{\PBRACK}[1]{\ensuremath{\left.\right\}\mathrel{\left[\,#1\,\right]}\left\{\right.}}

\newcommand{\ps}{\ensuremath{\boldsymbol{p}}}

\newcommand{\IFSYMBOL}{\ensuremath{\textnormal{\texttt{if}}}}
\newcommand{\IF}[1]{\ensuremath{\IFSYMBOL\,\left(\, {#1} \,\right)\,\{}}
\newcommand{\ELSESYMBOL}{\ensuremath{\textnormal{\texttt{else}}}}
\newcommand{\ELSE}{\ensuremath{\}\,\ELSESYMBOL\,\{}}
\newcommand{\ITE}[3]{\ensuremath{\IFSYMBOL\,\left(\, {#1} \,\right)\,\left\{\, {#2} \,\right\}\,\ELSESYMBOL\,\left\{\, {#3} \,\right\}}}

\newcommand{\WHILESYMBOL}{\ensuremath{\textnormal{\texttt{while}}}}
\newcommand{\WHILE}[1]{\ensuremath{\WHILESYMBOL \left(\, {#1} \,\right)}}

\newcommand{\WHILEDO}[2]{\ensuremath{\WHILESYMBOL \left(\, {#1} \,\right)\left\{\, {#2} \,\right\}}}



\newcommand{\Exp}{\ensuremath{\mathsf{Exp}}\xspace}
\newcommand{\e}{\ensuremath{f}}
\newcommand{\post}{\ensuremath{f}}
\newcommand{\pre}{\ensuremath{g}}
\newcommand{\postg}{\ensuremath{g}}
\newcommand{\posth}{\ensuremath{h}}

\newcommand{\wpsymbol}{\ensuremath{\mathsf{wp}}\xspace}
\renewcommand{\wp}[2]{\wpsymbol\,\llbracket#1\rrbracket\paren*{#2}}
\newcommand{\wpC}[1]{\wpsymbol\llbracket#1\rrbracket}
\newcommand{\wpVec}[2]{\smash{\overset{\text{\raisebox{-5pt}{$\longrightarrow$}}}{\wpsymbol}}\,\llbracket#1\rrbracket\paren*{#2}}

\newcommand{\VectDom}{\ensuremath{(\PosRealsInf)^n}} %
\newcommand{\MultDomFull}{\ensuremath{\Powerset{\VectDom}}} %
\newcommand{\MultDom}{\ensuremath{\PowerDown{\VectDom}}} 
\newcommand{\mExp}{\ensuremath{\mathsf{MultExp}}\xspace}
\newcommand{\me}{\ensuremath{\mathcal{F}}}
\newcommand{\mpost}{\ensuremath{\mathcal{F}}}
\newcommand{\meg}{\ensuremath{\mathcal{G}}}
\newcommand{\meset}{\ensuremath{\mathbb{F}}}
\newcommand{\mecup}{\ensuremath{\sqcup}}
\newcommand{\mmecup}{\morespace{\mecup}}
\newcommand{\bigmecup}{\ensuremath{\bigsqcup}}
\newcommand{\mecap}{\ensuremath{\sqcap}}
\newcommand{\mesubseteq}{\ensuremath{\sqsubseteq}}
\newcommand{\bigmecap}{\ensuremath{\bigsqcap}}
\newcommand{\mTrans}[1]{\ensuremath{\mathsf{M}[#1]}}

\newcommand{\mopsymbol}{\ensuremath{\mathsf{mop}}\xspace}
\newcommand{\mop}[2]{\mopsymbol\,\llbracket#1\rrbracket\paren*{#2}}
\newcommand{\mopC}[1]{\mopsymbol\llbracket#1\rrbracket}

\newcommand{\omopsymbol}{\ensuremath{\mathsf{omop}}}
\newcommand{\omop}[2]{\omopsymbol\,\llbracket#1\rrbracket\paren*{#2}}
\newcommand{\omopC}[1]{\omopsymbol\llbracket#1\rrbracket}

\newcommand{\programdeterm}{\ensuremath{\program^d}}


\newcommand{\entails}{\models}
\newcommand{\eentails}{\morespace{\entails}}
\newcommand{\qentails}{\qmorespace{\entails}}
\newcommand{\qqentails}{\qqmorespace{\entails}}
\newcommand{\Exec}[6]{\ensuremath{\step{#1,#2}{#3, #4}{#5, #6} }}

\newcommand{\qmid}{\quad{}|{}\quad}
\newcommand{\ttsymbol}[1]{\texttt{\upshape {#1}}}
\newcommand{\setcomp}[2]{\left\{\, {#1} ~\middle|~ {#2} \,\right\}}
\newcommand{\subst}[2]{\left[ {#1} \middle/ {#2}\right]}
\newcommand{\substState}[3]{#1 \left[ #2 \mapsto #3\paren*{#1} \right]}

\newcommand*\oline[1]{%
  \vbox{%
    \hrule height 0.3pt%
    \kern0.25ex%
    \hbox{%
      \kern0.04em%
      \ifmmode#1\else\ensuremath{#1}\fi%
      \kern0.04em%
    }%
  }%
}

\newcommand{\negate}[1]{\neg #1}	
\newcommand{\mydot}{\text{{\Large\textbf{.}}~}\xspace}
\newcommand{\mylambda}[1]{\lambda\, #1\mydot}


\newcommand{\lfp}{\ensuremath{\textnormal{\textsf{lfp}}~}}
\newcommand{\gfp}{\ensuremath{\textnormal{\textsf{gfp}}~}}




\newcommand{\OpConf}{\ensuremath{\mathsf{Conf}}}
\newcommand{\OpP}{\ensuremath{\mathsf{P}}}
\newcommand{\OpStates}{\ensuremath{S}}
\newcommand{\OpStatesN}{\ensuremath{\OpStates_N}}
\newcommand{\OpStatesP}{\ensuremath{\OpStates_P}}
\newcommand{\OpAct}{\ensuremath{\mathsf{Act}}}
\newcommand{\OpRew}{\ensuremath{\mathsf{rew}}}
\newcommand{\OpRewCast}{\ensuremath{\OpRew_c}}
\newcommand{\OpSucc}{\ensuremath{\mathsf{Succ}}}
\newcommand{\OpNondet}{\ensuremath{\mathsf{ND}}}
\newcommand{\OpStrat}[2]{\ensuremath{\mathsf{Str}_{#1}^{#2}}} %

\newcommand{\opState}{\ensuremath{s}}
\newcommand{\opAct}{\ensuremath{\mathsf{a}}}
\newcommand{\opConf}{\ensuremath{\mathsf{c}}}

\newcommand{\ex}[2]{\ensuremath{\mathrm{Ex}_{#1}^{#2}}}  %
\newcommand{\ExpRew}[4]{\ensuremath{\mathsf{ExpRew}^{#1,#2}_{#3,#4}}}  %
\newcommand{\ExpRewN}[4]{\ensuremath{\mathsf{ExpRew}[k]^{#1,#2}_{#3,#4}}}  %
\newcommand{\ExpRewI}[5]{\ensuremath{\mathsf{ExpRew}[#5]^{#1,#2}_{#3,#4}}}  %
\newcommand{\MaxExpRew}[3]{\ensuremath{\mathsf{MaxExpRew}^{#1,#2}_{#3}}}  %
\newcommand{\MaxExpRewN}[3]{\ensuremath{\mathsf{MaxExpRew}[k]^{#1,#2}_{#3}}}  %
\newcommand{\AchExpRew}[3]{\ensuremath{\mathsf{AchExpRew}^{#1,#2}_{#3}}}  %
\newcommand{\AchExpRewN}[3]{\ensuremath{\mathsf{AchExpRew}[k]^{#1,#2}_{#3}}}  %

 
\newcommand{\AchEx}[3]{\ensuremath{\mathsf{AchEx}^{#1,#2}_{#3}}}  %
\newcommand{\Ach}[3]{\ensuremath{\mathsf{Ach}^{#1,#2}_{#3}}}  %
\newcommand{\AchMemless}[3]{\ensuremath{\mathsf{AchMemless}^{#1,#2}_{#3}}}  %
\newcommand{\AchFin}[3]{\ensuremath{{\bigcup_{k \in \Nats} \AchN{#1}{#2}{#3}}}}  %
\newcommand{\Pareto}[3]{\ensuremath{\mathsf{Pareto}^{#1,#2}_{#3}}}  %
\newcommand{\ParetoOpt}[3]{\ensuremath{\mathsf{ParetoOpt}^{#1,#2}_{#3}}}  %

\newcommand{\ParetoMDP}[1]{\ensuremath{\mathsf{Pareto}^{#1}}}  %
\newcommand{\AchMDP}[1]{\ensuremath{\mathsf{Ach}^{#1}}}  %

\newcommand{\AchExp}[3]{\ensuremath{\mathsf{Ach}^{#1,#2}_{#3}}}  %
\newcommand{\ParetoExp}[3]{\ensuremath{\mathsf{Pareto}^{#1,#2}_{#3}}}  %

\newcommand{\AchExN}[3]{\ensuremath{\mathsf{AchEx}[k]^{#1,#2}_{#3}}}  %
\newcommand{\AchN}[3]{\ensuremath{\mathsf{Ach}[k]^{#1,#2}_{#3}}}  %
\newcommand{\AchI}[4]{\ensuremath{\mathsf{Ach}[#4]^{#1,#2}_{#3}}}  %
\newcommand{\ParetoN}[3]{\ensuremath{\mathsf{Pareto}[k]^{#1,#2}_{#3}}}  %
\newcommand{\ParetoOptN}[3]{\ensuremath{\mathsf{ParetoOpt}[k]^{#1,#2}_{#3}}}  %


\newcommand{\finPaths}[1]{\ensuremath{\mathsf{Paths}_{\mathsf{fin}}^{#1}}}
\newcommand{\finPath}{\ensuremath{\hat{\pi}}}
\newcommand{\nPaths}[1]{\ensuremath{\mathsf{Paths}_{k}^{#1}}}
\newcommand{\mPaths}[1]{\ensuremath{\mathsf{Paths}_{l}^{#1}}}
\newcommand{\iPaths}[2]{\ensuremath{\mathsf{Paths}_{#2}^{#1}}}
\newcommand{\nPath}{\ensuremath{\hat{\pi_k}}}
\newcommand{\lnPaths}[1]{\ensuremath{\mathsf{Paths}_{\leq k}^{#1}}}
\newcommand{\lnPath}{\ensuremath{\hat{\pi_{\leq k}}}}
\newcommand{\infPaths}[1]{\ensuremath{\mathsf{Paths}_{\mathsf{inf}}^{#1}}}
\newcommand{\infPath}{\ensuremath{\pi}}
\newcommand{\last}[1]{\ensuremath{\mathsf{last}\paren*{#1}}}

\newcommand{\pathProb}[2]{\ensuremath{\mathsf{Prob}^{#1}_{#2}}} %

\newcommand{\RewDom}{\ensuremath{D}}  
\newcommand{\RewDomMax}{\ensuremath{\PosRealsInf}}  
\newcommand{\RewDomPareto}{\ensuremath{\PowerDown{(\PosRealsInf)^n}}}  

\newcommand{\distr}[1]{\ensuremath{\mathsf{Dist}}\paren*{#1}}

\newcommand{\Sched}[1]{\ensuremath{\mathsf{Sched}}^{#1}}
\newcommand{\sched}{\ensuremath{\rho}}
\newcommand{\SchedPure}[1]{\ensuremath{\mathsf{Sched}_P^{#1}}}
\newcommand{\SchedMemless}[1]{\ensuremath{\mathsf{SchedMemless}^{#1}}}
\newcommand{\SchedSimple}[1]{\ensuremath{\mathsf{Sched}_S^{#1}}}
\newcommand{\SchedMemfull}[1]{\ensuremath{\mathsf{Sched}_M^{#1}}}

\newcommand{\Bellman}[2]{\ensuremath{\Phi^{#1}_{#2}}}
\newcommand{\BellmanNo}{\ensuremath{\Phi}}

\newcommand{\mBellman}[2]{\ensuremath{\Omega^{#1}_{#2}}}
\newcommand{\mBellmanNo}{\ensuremath{\Omega}}

\newcommand{\mdBellman}[2]{\ensuremath{\widehat{\Omega}^{#1}_{#2}}}
\newcommand{\mdBellmanNo}{\ensuremath{\widehat{\Omega}}}

\newcommand{\BellmanMax}[2]{\ensuremath{{^{\mathsf{max}}_{#1}\Phi_{#2}}}}
\newcommand{\BellmanPareto}[2]{\ensuremath{{^{\mathsf{Ach}}_{#1}\Phi_{#2}}}}
\newcommand{\BellmanParetoNo}{\ensuremath{{^{\mathsf{Ach}}\Phi}}}


\newcommand{\V}{\ensuremath{\mathbb{V}}}
\newcommand{\MV}{\ensuremath{\mathbb{MV}}}
\newcommand{\mv}{\ensuremath{V}}
\newcommand{\MVdown}{\ensuremath{\mathbb{MV}_\downarrow}}

\newcommand{\Vleq}{\ensuremath{\leq}}
\newcommand{\MVleq}{\ensuremath{\leq}}

\newcommand{\MDP}{\ensuremath{\mathcal{M}}}
\newcommand{\ProgM}[1]{\ensuremath{\MDP \llbracket #1 \rrbracket}}
\newcommand{\ProgMDP}{\ensuremath{\mathcal{O}}}
\newcommand{\ProgR}[1]{\ensuremath{\OpRew \llbracket #1 \rrbracket}}

\newcommand{\step}[3]{#1 \,\xrightarrow{#2}\, #3}

\newcommand{\minkow}{\ensuremath{\oplus}}
\newcommand{\mminkow}{\morespace{\minkow}}
\newcommand{\qminkow}{\qmorespace{\minkow}}
\newcommand{\qqminkow}{\qqmorespace{\minkow}}
\newcommand{\Minkow}{\ensuremath{\bigoplus}}

\newcommand{\bighoaresup}{\ensuremath{\bigsqcup}}
\newcommand{\hoaresup}{\ensuremath{\sqcup}}
\newcommand{\hoareinf}{\ensuremath{\sqcap}}
\newcommand{\bighoareinf}{\ensuremath{\bigsqcap}}

\newcommand{\annocolor}[1]{\textcolor{DarkOrange3}{#1}}
\newcommand{\annotate}[1]{\boldsymbol{\annocolor{\!\fatslash\!\!\!\fatslash~~\vphantom{G'} {#1}}}}
\newcommand{\annotateNo}[1]{\boldsymbol{\annocolor{\phantom{\!\fatslash\!\!\!\fatslash~~}\vphantom{G'} {#1}}}}

\newcommand{\vvec}[2]{\left(\begin{smallmatrix}#1\\#2\end{smallmatrix}\right)}
\newcommand{\vvvec}[3]{\left(\begin{smallmatrix}#1\\#2\\#3\end{smallmatrix}\right)}
\newcommand{\vvechorizon}[2]{\left(#1,\, #2\right)}
\newcommand{\vvvechorizon}[3]{\left(#1,\, #2,\, #3\right)}



\newcommand{\cheat}[1]{\ensuremath{\dblbrace{#1}}} 

\newcommand{\determ}{\ensuremath{\multimap}}

\newcommand{\determopt}[1]{%
  \mathrel{%
    \tikz[baseline=-0.6ex]{
      \draw[line width=0.4pt] (0,0) -- (1.6em,0);
      \draw (1.7em,0) circle (0.3ex);
      \node[font=\tiny,anchor=south,yshift=-1.1ex,color=gray] at (0.75em,0) {$\mathrm{opt}$};
      \node[font=\tiny,anchor=north,yshift=0.7ex,color=gray] at (0.75em,0) {$#1$};
    }%
  }%
}

\newcommand{\ddeterm}{\morespace{\determ}}
\newcommand{\hqdeterm}{\hqmorespace{\determ}}
\newcommand{\qdeterm}{\qmorespace{\determ}}
\newcommand{\qqdeterm}{\qqmorespace{\determ}}
\usetikzlibrary{decorations.pathmorphing}

\newcommand{\squigglymultimap}{%
  \mathrel{\tikz[baseline=-0.5ex]{
    \draw[decorate,decoration={snake,amplitude=.6pt,segment length=3pt}]
      (0,0) -- (0.9em,0);
    \draw (1em,0) circle (.12em);
  }}
}
\newcommand{\determmixed}{\ensuremath{\squigglymultimap}}

\newcommand{\Vals}{\ensuremath{\mathsf{Vals}}\xspace}  

\newcommand{\EVT}[3]{\ensuremath{\mathsf{EVT}_{#1}^{#2}{\paren*{#3}}}\xspace}  %

\newcommand{\phiMopNo}{\ensuremath{\Phi^{\mopsymbol}}}
\newcommand{\molpsymbol}{\ensuremath{\mathsf{molp}}\xspace}
\newcommand{\molp}[2]{\molpsymbol\,\llbracket#1\rrbracket\paren*{#2}}
\newcommand{\molpC}[1]{\molpsymbol\llbracket#1\rrbracket}
\newcommand{\phiMolpNo}{\ensuremath{\Phi^{\molpsymbol}}}
\newcommand{\topME}{\ensuremath{\boldsymbol{\top}}} %
\newcommand{\phiMop}[2]{\ensuremath{_{#1}\Phi^{\mopsymbol}_{#2}}}
\newcommand{\phiWp}[2]{\ensuremath{_{#1}\Phi^{\wpsymbol}_{#2}}}
\newcommand{\phiWpNo}{\ensuremath{\Phi^{\wpsymbol}}}


\newcommand{\zeroHoare}{\ensuremath{\boldsymbol{0}}}
\newcommand{\zeroMV}{\ensuremath{\boldsymbol{0}}}
\newcommand{\zeroME}{\ensuremath{\boldsymbol{0}}}


\newcommand{\dblbrace}[1]{%
  \mathinner{\{\mkern-3.5mu\vert#1\vert\mkern-3.5mu\}}%
}

\newcommand{\weight}{\ensuremath{w}} %
\newcommand{\weightc}{\ensuremath{\lambda}} %
\newcommand{\Weights}{\ensuremath{W}}
\newcommand{\HDel}{\ensuremath{H}} %
\newcommand{\scal}[2]{\ensuremath{#1 \odot #2}} %



\newcommand{\multiguard}{\ensuremath{\boldsymbol{\varphi}\vert\determVar}} %
\newcommand{\determVar}{\ensuremath{\xi}} %
\newcommand{\determDist}{\ensuremath{\Pi}} %


\newcommand{\GCARROW}{\shortrightarrow}
\newcommand{\ENDIFSYMBOL}{}
\newcommand{\GC}[4]{\ensuremath{\IFSYMBOL\hspace*{.5em}{#1}\GCARROW\{{#2}\} \hqmorespace{\square}{#3}\GCARROW\{{#4}\}\ENDIFSYMBOL}} %
\newcommand{\GCFST}[2]{\ensuremath{\IFSYMBOL\,{#1}\GCARROW\{{#2}\}}}
\newcommand{\GCFSTOPEN}[1]{\ensuremath{\IFSYMBOL\,{#1}\GCARROW\{ }}
\newcommand{\GCFSTCLOSE}{\ensuremath{\}}}
\newcommand{\GCSEC}[2]{\ensuremath{{~{}\square{}~}\hspace{0.015cm}{#1}\GCARROW\{{#2}\}\,\ENDIFSYMBOL}}
\newcommand{\GCSECOPEN}[1]{\ensuremath{{~{}\square{}~}\hspace{0.015cm}{#1}\GCARROW\{ }}
\newcommand{\GCSECCLOSE}{\ensuremath{\} \ENDIFSYMBOL}}


\newcommand{\ppreceq}{~{}\preceq{}~}
\newcommand{\ssucceq}{~{}\succeq{}~}
\newcommand{\eeq}{~{}={}~}
\newcommand{\defeq}{\coloneqq}
\newcommand{\ddefeq}{~{}\coloneqq{}~}
\newcommand{\neeq}{~{}\neq{}~}
\newcommand{\qeq}{\quad{}={}\quad}
\newcommand{\qqeq}{\qquad{}={}\qquad}
\newcommand{\lleq}{~{}\leq{}~}
\newcommand{\LL}{~{}<{}~}
\newcommand{\ggeq}{~{}\geq{}~}
\newcommand{\ssqsubseteq}{~{}\sqsubseteq{}~}
\newcommand{\qsqsubseteq}{\qmorespace{\sqsubseteq}}
\newcommand{\qqsqsubseteq}{\qqmorespace{\sqsubseteq}}
\newcommand{\ssqcup}{\morespace{\sqcup}}
\newcommand{\pplus}{\morespace{+}}
\newcommand{\iimplies}{~{}\implies{}~}
\newcommand{\mmodels}{~{}\models{}~}
\newcommand{\nnotmodels}{~{}\not\models{}~}
\newcommand{\iin}{~{}\in{}~}
\newcommand{\nnotin}{~{}\not\in{}~}
\newcommand{\morespace}[1]{~{}#1{}~}
\newcommand{\hqmorespace}[1]{\hspace*{.5em}{}#1{}\hspace*{.5em}}
\newcommand{\qmorespace}[1]{\quad{}#1{}\quad}
\newcommand{\qqmorespace}[1]{\qquad{}#1{}\qquad}
\newcommand{\ttimes}{\morespace{\times}}
\newcommand{\lland}{\morespace{\land}}
\newcommand{\llor}{\morespace{\lor}}

\newcommand{\qiff}{\qmorespace{\textnormal{ iff }}}
\newcommand{\qqiff}{\qqmorespace{\textnormal{ iff }}}

\newcommand{\aand}{\morespace{\textnormal{ and }}}
\newcommand{\qand}{\qmorespace{\textnormal{ and }}}
\newcommand{\qqand}{\qqmorespace{\textnormal{ and }}}

\newcommand{\aor}{\morespace{\textnormal{ or }}}
\newcommand{\qor}{\qmorespace{\textnormal{ or }}}
\newcommand{\qqor}{\qqmorespace{\textnormal{ or }}}

\newcommand{\expecs}{\mathbb{E}} %
\newcommand{\expecsbnd}[1]{\expecs_{\leq #1}} %
\newcommand{\predicates}{\mathbb{P}} %
\newcommand{\expclass}{\Xi}


\newcommand{\WHILEDOINV}[3]{\WHILEDOINVOPEN{#1} {#2} \WHILEDOINVCLOSE{#3}}
\newcommand{\WHILEDOINVOPEN}[1]{\WHILESYMBOL\,{#1}\GCARROW\{}
\newcommand{\WHILEDOINVCLOSE}[1]{\}\,\langle#1\rangle\,\ENDWHILESYMBOL}

\newcommand{\inv}{\invariant}

\newcommand{\ENDWHILESYMBOL}{}


\newcommand{\ExecSymbol}{\ensuremath{\rightarrow}}
\newcommand{\mc}{t}
\newcommand{\msched}{\sched}
\newcommand{\MSCHED}{\mathit{Strats}}
\newcommand{\MSCHEDMD}{\MSCHED^{MD}}
\newcommand{\supp}[1]{\mathit{supp}\paren*{#1}} %

\newcommand{\MI}{\OpStates_{\textnormal{\text{init}}}}
\newcommand{\MT}{T} %

\newcommand{\MG}{G} %
\newcommand{\pathstotarget}[1]{{\mathlarger{\lozenge}}#1}
\newcommand{\probofpath}[2]{\textnormal{\textsf{Prob}}_{#1}\left( #2 \right)}
\newcommand{\exprew}[3]{\textnormal{\textsf{ExpRew}}_{#1}\llbracket #2 \rrbracket\left(#3\right)}
\newcommand{\exprewmc}[2]{\textnormal{\textsf{ExpRew}}_{}\llbracket #1 \rrbracket\left(#2\right)}
\newcommand{\minexprew}[2]{\textnormal{\textsf{MinExpRew}}_{}\llbracket #1 \rrbracket\left(#2\right)}
\newcommand{\maxexprew}[2]{\textnormal{\textsf{MaxExpRew}}_{}\llbracket #1 \rrbracket\left(#2\right)}
\newcommand{\thresh}{\rho}

\newcommand{\mi}{\opState_{\textnormal{\text{init}}}}





\newcommand{\face}[2]{\ensuremath{\mathsf{face}\paren*{#1,#2} }}

\newcommand{\DetermSimple}[1]{\ensuremath{\textsf{DetPure}\paren*{#1}}}
\newcommand{\DetermMixed}[1]{\ensuremath{\textsf{Det}\paren*{#1}}}


\newcommand{\monus}{\ensuremath{\mathbin{\dot{-}}}}


\newcommand{\xor}{\ensuremath{\veebar}} %
\newcommand{\myendmark}{\hfill\gray{$\triangleleft$}}



\newcommand{\PCHOICEFINITE}[4]{\ensuremath{\set{#1}_{#2}[#3]_{#4}}}
\newcommand{\SampleSymbol}{\mathrel{\vcentcolon\approx}}
\newcommand{\SAMPLE}[2]{\ensuremath{#1 \SampleSymbol #2}}


\newcommand{\finval}{\ensuremath{\ll}}


\newcommand{\infer}[2]{\frac{#2}{#1}}

\newcommand{\programrun}{\ensuremath{\program_{\text{run}}}}


\newcommand{\qf}{\ensuremath{q_{\mathrm{f}}}}
\newcommand{\qs}{\ensuremath{q_{\mathrm{s}}}}
\newcommand{\gap}{\ensuremath{g}}
\newcommand{\leanname}[1]{\texttt{#1}}

\newcommand{\invariant}{\ensuremath{I}}



\definecolor{mylightgreen}{RGB}{140,185,132} %
\definecolor{mygreen}{RGB}{85,140,75}
\definecolor{myblue}{RGB}{53,121,245}
\definecolor{myred}{RGB}{185,49,34}

\newcommand{\orange}[1]{\textcolor{orange}{#1}}
\newcommand{\red}[1]{\textcolor{myred}{#1}}
\newcommand{\blue}[1]{\textcolor{myblue}{#1}}
\newcommand{\gray}[1]{\textcolor{gray}{#1}} %

\newcommand{\target}{\ensuremath{\tau}} 


\newcommand{\bd}[1]{\ensuremath{\mathit{bd}\paren*{#1}}} 

\newcommand{\argmax}{\ensuremath{\mathsf{argmax}}} 

\newcommand{\sem}[2]{\ensuremath{\llbracket {#1} \rrbracket}(#2)}



\newcommand{\titleCref}[1]{\texorpdfstring{\Cref{#1}}{Theorem~\ref{#1}}}

\newcommand{\extreme}[1]{\ensuremath{\mathit{Ext}\paren*{#1}}}
\newcommand{\exposed}[1]{\ensuremath{\mathit{Exp}\paren*{#1}}}

